Inverse Superconductor-Insulator Transition in Weakly Monitored Josephson Junction Arrays

Control and manipulation of quantum states by measurements and bath engineering in open quantum systems have emerged as new paradigms in many-body physics. Here, taking a prototypical example of Josephson junction arrays (JJAs), we show how repetitive monitoring through continuous weak measurements and feedback can transform an insulating state in these systems to a superconductor and vice versa. We show that, even in the absence of any external thermal bath, the monitoring leads to a long-time steady state characterized by an effective `quantum' temperature in a suitably defined semiclassical limit. However, we show that the quantum dissipation due to monitoring has fundamental differences with equilibrium quantum and/or thermal dissipation in the well-studied case of JJAs in contact with an Ohmic bath. In particular, using a variational approximation, and by considering various limiting cases, we demonstrate that this difference can give rise to re-entrant steady-state phase transitions, resulting in unusual inverse transition from an effective low-temperature insulating normal state to superconducting state at intermediate temperature. Our work emphasizes the role of quantum feedback, that acts as an additional knob to control the effective temperature of non-equilibrium steady state leading to a phase diagram, not explored in earlier works on monitored and open quantum systems.

==> definitions.tex <==
%-----------------For nomenclature ------------------
\newcommand{\usenomenclature}{}
\ifdefined\usenomenclature
\usepackage[noprefix]{nomencl}
\fi
\newcommand{\makenomcl}{\ifdefined\usenomenclature\makenomenclature\fi}
%\newcommand{\makenomcl}{\makenomenclature}
\newcommand{\nomcl}[2]{\ifdefined\usenomenclature \nomenclature{#1}{#2}\fi}
\newcommand{\nomcls}[3]{\ifdefined\usenomenclature \nomenclature[#1]{#2}{#3}\fi}

%\newcommand{\nomcl}[2]{\nomenclature{#1}{#2}}
\newcommand{\printnomcl}{\ifdefined\usenomenclature\printnomenclature\fi}
%\newcommand{\printnomcl}{\printnomenclature}
\newcommand{\symref}[1]{First appearance in sec~\ref{#1}, page \pageref{#1}.}
\newcommand{\symeqref}[1]{First appearance in \eqn{#1}, page \pageref{#1}.}
\newcommand{\symdefref}[1]{Defined in \eqn{#1}, page \pageref{#1}.}

%----------From SREP mauscript------------
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
%\newcommand{\eqn}[1] {equation~(\ref{#1})}
\newcommand{\Eqn}[1] {Eqn.~(\ref{#1})}
\newcommand{\eqn}[1] {eqn.~(\ref{#1})}
\newcommand{\eqnSM}[1] {eqn.~(\ref{#1})}
\newcommand{\prn}[1] {(\ref{#1})}
\newcommand{\sect}[1] {Section~\ref{#1}}
\newcommand{\Seccite}[1] {Sec.~\ref{#1}}
\newcommand{\fig}[1]{fig.~\ref{#1}}
\newcommand{\figSM}[1]{fig.~\ref{#1}}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\FigSM}[1]{Fig.~\ref{#1}}
%\newcommand{\ttd}[1]{{\color[rgb]{1,0,0}{\bf #1}}}
%\newcommand{\ttd}[1]{{\color[rgb]{1,0,0}{#1}}}
\newcommand{\ttd}[1]{#1}
%set this to see the name of the labels in the margins
%\setlength{\textwidth}{15truecm}
%\newcommand{\mylabel}[1]{\label{#1}	{\marginnote[\footnotesize{\tt #1}]%{\footnotesize{\tt #1}}}}

%
%or this for doing nothing
\newcommand{\mylabel}[1]{\label{#1}} 
\newcommand{\mycite}[1]{\cite{#1}}
%------------------------------------------

%----------From SHMMISYK-------------------
%%my definitions
\newcommand{\bcen}{\begin{center}}
\newcommand{\ecen}{\end{center}}
\newcommand{\btab}{\begin{tabular}}
\newcommand{\etab}{\end{tabular}}
\newcommand{\bdes}{\begin{description}}
\newcommand{\edes}{\end{description}}
\newcommand{\mc}{\multicolumn}
\newcommand{\ul}{\underline}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\non}{\nonumber}
\newcommand{\etal}{et.~al.\ }
\newcommand{\half}{\frac{1}{2}}
\newcommand{\bary}{\begin{array}}
\newcommand{\eary}{\end{array}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}
\newcommand{\cuup}[1]{c_{#1 \uparrow}}
\newcommand{\cdown}[1]{c_{#1 \downarrow}}
\newcommand{\cdup}[1]{c^\dagger_{#1 \uparrow}}
\newcommand{\cddown}[1]{c^\dagger_{#1 \downarrow}}
%
%bold greek characters
%
\newcommand{\beps}{\mbox{\boldmath $ \epsilon $}}
\newcommand{\bsig}{\mbox{\boldmath $ \sigma $}}
\newcommand{\bpi}{\mbox{\boldmath $ \pi $}}
\newcommand{\bkap}{\mbox{\boldmath $ \kappa $}}
\newcommand{\bgam}{\mbox{\boldmath $ \gamma $}}
\newcommand{\bphi}{\mbox{\boldmath $ \phi $}}
\newcommand{\balp}{\mbox{\boldmath $ \alpha $}}
\newcommand{\beot}{\mbox{\boldmath $ \eta $}}
\newcommand{\btau}{\mbox{\boldmath $ \tau $}}
\newcommand{\blam}{{\boldsymbol{\lambda}}}
\newcommand{\bomg}{\mbox{\boldmath $ \omega $}}
\newcommand{\bOmg}{\mbox{\boldmath $ \Omega $}}
\newcommand{\bxhi}{\mbox{\boldmath $ \xi $}}
\newcommand{\bmu} {\mbox{\boldmath $ \mu $}}
\newcommand{\bnu} {\mbox{\boldmath $ \nu $}}
\newcommand{\bdelta}{{\boldsymbol{\delta}}}
\newcommand{\bDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bPi}{{\boldsymbol{\Pi}}}
\newcommand{\bpsi}{\mbox{\boldmath $ \psi $}}
\newcommand{\brho}{\mbox{\boldmath $ \rho $}}
\newcommand{\bGam}{{\boldsymbol{\Gamma}}}
\newcommand{\bLam}{\mbox{\boldmath $ \Lambda $}}
\newcommand{\bPhi}{\mbox{\boldmath $ \Phi $}}
\newcommand{\bOne}{{\boldsymbol 1}}
%
%bold latin
%
%\newcommand{\ba} { \mbox{\boldmath $a$}}
\newcommand{\ba} { \bm{a} }
\newcommand{\bb} { \mbox{\boldmath $b$}}
%\newcommand{\bc} { \mbox{\boldmath $c$}}
\newcommand{\bc} { {\mathbf c} }
\newcommand{\bd} { \mbox{\boldmath $d$}}
\newcommand{\be} { \mbox{\boldmath $e$}}
\newcommand{\bff}{ \mbox{\boldmath $f$}}
\newcommand{\bg} { \mbox{\boldmath $g$}}
\newcommand{\bh} { \mbox{\boldmath $h$}}
\newcommand{\bi} { \mbox{\boldmath $i$}}
\newcommand{\bj} { \mbox{\boldmath $j$}}
\newcommand{\bk} { \bm{k} }
%\newcommand{\bk} { \mbox{\boldmath $k$}}
\newcommand{\bl} { \mbox{\boldmath $l$}} 
\newcommand{\bmm} { \mbox{\boldmath $m$}}
\newcommand{\bn} { \mbox{\boldmath $n$}}
\newcommand{\bo} { \mbox{\boldmath $o$}}
\newcommand{\bp} { \bm{p} }
\newcommand{\bq} { \bm{q} }
%\newcommand{\bq} { \mbox{\boldmath $q$}}
\newcommand{\br} { \boldsymbol{r}}
\newcommand{\bs} { \mbox{\boldmath $s$}}
\newcommand{\bt} {\boldsymbol{t}} 
\newcommand{\bu} { \mbox{\boldmath $u$}}
\newcommand{\bv} { \mbox{\boldmath $v$}}
\newcommand{\bw} { \mbox{\boldmath $w$}}
\newcommand{\bx} { \mbox{\boldmath $x$}}
\newcommand{\by} { \mbox{\boldmath $y$}}
\newcommand{\bz} { \mbox{\boldmath $z$}}

\newcommand{\bA} { \mbox{\boldmath $A$}}
\newcommand{\bB} { \mbox{\boldmath $B$}}
\newcommand{\bC} { \mbox{\boldmath $C$}}
\newcommand{\bD} { \mbox{\boldmath $D$}}
\newcommand{\bE} { \mbox{\boldmath $E$}}
\newcommand{\bF} { \mbox{\boldmath $F$}}
\newcommand{\bG} { \mbox{\boldmath $G$}}
\newcommand{\bH} { \mbox{\boldmath $H$}}
\newcommand{\bI} { \mbox{\boldmath $I$}}
\newcommand{\bJ} { \mbox{\boldmath $J$}}
\newcommand{\bK} { \mbox{\boldmath $K$}}
\newcommand{\bL} { \mbox{\boldmath $L$}}
\newcommand{\bM} { \mbox{\boldmath $M$}}
\newcommand{\bN} { \mbox{\boldmath $N$}}
\newcommand{\bO} { \mbox{\boldmath $O$}}
\newcommand{\bP} { \mbox{\boldmath $P$}}
\newcommand{\bQ} { \boldsymbol{Q} }
%\newcommand{\bQ} { \mbox{\boldmath $Q$}}
\newcommand{\bR} { {\mathbf R} }
%\newcommand{\bR} { \mbox{\boldmath $R$}}
\newcommand{\bS} { \mbox{\boldmath $S$}}
\newcommand{\bT} { \mbox{\boldmath $T$}}
\newcommand{\bU} { \mbox{\boldmath $U$}}
\newcommand{\bV} { \mbox{\boldmath $V$}}
\newcommand{\bW} { \mbox{\boldmath $W$}}
\newcommand{\bX} { \mbox{\boldmath $X$}}
\newcommand{\bY} { \mbox{\boldmath $Y$}}
\newcommand{\bZ} { \mbox{\boldmath $Z$}}
\newcommand{\bzero} { {\boldsymbol{0}}}
\newcommand{\bfell} {\mbox{\boldmath $ \ell $}}

%
%special math symbols
%
\newcommand{\dou}{\partial}
\newcommand{\leftjb} {[\![}
\newcommand{\rightjb} {]\!]}
\newcommand{\ju}[1]{ \leftjb #1 \rightjb }
\newcommand{\D}[1]{\mbox{d}{#1}} 
\newcommand{\grad}{\mbox{\boldmath $\nabla$}}
\newcommand{\modulus}[1]{|#1|}
\renewcommand{\div}[1]{\grad \cdot #1}
\newcommand{\curl}[1]{\grad \times #1}
\newcommand{\mean}[1]{\langle #1 \rangle}
\newcommand{\bra}[1]{{\langle #1 |}}
\newcommand{\ket}[1]{| #1 \rangle}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\dbdou}[2]{\frac{\dou #1}{\dou #2}}
\newcommand{\dbdsq}[2]{\frac{\dou^2 #1}{\dou #2^2}}
\newcommand{\Pint}[2]{ P \!\!\!\!\!\!\!\int_{#1}^{#2}}

\newcommand{\PARA}[1]{{\noindent {$\bigstar$} {\sc #1}:~}}
\newcommand{\paratitle}[1]{\noindent {\bf #1:}}

%abbreviations for equations etc
% 
\newcommand \SMcite[1]{\mycite{SM}, \ref{#1}}
\newcommand \SMsubcite[1]{\mycite{SM}, \ref{#1}}
\newcommand \seccite[1]{sec.~\ref{#1}}
\newcommand{\pararef}[1]{para \ref{#1}}


%
% Roman Numerals
%
\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

%
%Other utilities
%
\newcommand{\uncon}[1]{\centerline{\epsfysize=#1 \epsfbox{/usr2/shenoy/styles/construction.eps}}}
\newcommand{\checkup}[1]{{(\tt #1)}\typeout{#1}}
\newcommand{\ttds}[1]{{\color[rgb]{0,0,1}{\bf #1}}}
\newcommand{\red}[1]{{\color[rgb]{1,0,0}{\protect{#1}}}}
\newcommand{\blue}[1]{{\color[rgb]{0,0,1}{#1}}}
\newcommand{\green}[1]{{\color[rgb]{0.0,0.5,0.0}{#1}}}
\newcommand{\brickred}[1]{{\color[rgb]{0.61,0.12,0.11}{#1}}}
\newcommand{\citebyname}[1]{\citeauthor{#1}\cite{#1}}
\newcommand{\signum}[0]{\mathop{\mathrm{sign}}}
\newcommand{\skup}{\ket{s \uparrow}}
\newcommand{\skdn}{\ket{s \downarrow}}
\newcommand{\pkup}{\ket{p \uparrow}}
\newcommand{\pkdn}{\ket{p \downarrow}}
\newcommand{\sbup}{\bra{s \uparrow}}
\newcommand{\sbdn}{\bra{s \downarrow}}
\newcommand{\pbup}{\bra{p \uparrow}}
\newcommand{\pbdn}{\bra{p \downarrow}}

%width of figures
\newcommand{\myfigwidth}{0.99\columnwidth}
\newcommand{\myhalffigwidth}{0.495\columnwidth}


\newcommand{\asc}{a_{sc}}
\newcommand{\as}{a_{s}}
\newcommand{\Eb}{E_{b}}
\newcommand{\Ef}{E_F}
\newcommand{\kf}{k_F}
\newcommand{\lambdaT}{{\lambda_T}}
\newcommand{\cF}{{\cal F} }
\newcommand{\ie}{{i.e., } }
\newcommand{\etaT}{{\eta_t}}
\newcommand{\muNI}{{\mu_{NI}}}

%set this to see the name of the labels in the margins
%\newcommand{\mylabel}[1]{\label{#1}{\marginnote{\tiny{\tt #1}}}}
%
%or this for this for doing nothing
\newcommand{\citewithfile}[2]{\cite{#2}\href{./#1}{File}}
%\newcommand{\myonlinecite}[1]{[\onlinecite{#1}]}
%\newcommand{\mycite}[1]{$\tt{#1}$\cite{#1}}


\newcommand{\authornat}[2]{\author{#1$^*$ \\ $^*$email: #2}}
\newcommand{\authorprl}[2]{\author{#1}\email{#2}}
\newcommand{\authornoemail}[2]{\author{#1}}

%\renewcommand{\hline}{\midrule}
%\setlength{\midrulewidth}{0.1 em}
%%STUFFforlinenumbers
%\usepackage{lineno}
%\setpagewiselinenumbers
%\modulolinenumbers[5]
%\linenumbers

% You should use BibTeX and   apsrev.bst for references
%nd{\citewithfile}[2]{\cite{#2}\href{./#1}{File}} Choosing a journal automatically selects the correct APS
% BibTeX style file (bst file), so only uncomment the line
% below if necessary.

\DeclareMathOperator{\sgn}{sgn}

\newcommand{\BA}{BA}
\newcommand{\qs}{{q_s}}
\newcommand{\qc}{{q_c}}
\newcommand{\qPsi}{{q_\Psi}}
\newcommand{\Lo}{{N}}
\newcommand{\Lc}{{N}}
\newcommand{\LPsi}{{M}}
\newcommand{\Tc}{{Q_c}}
\newcommand{\Jc}{{J_c}}
\newcommand{\JPsi}{{J_\Psi}}
\newcommand{\TPsi}{{Q_\Psi}}
\newcommand{\Pc}{{P_c}}
\newcommand{\PPsi}{{P_\Psi}}
\newcommand{\Gc}{{G_c}}
\newcommand{\GPsi}{{G_\psi}}
\newcommand{\Sigc}{{\Sigma_c}}
\newcommand{\SigPsi}{{\Sigma_\psi}}
\newcommand{\fx}{f}
\newcommand{\ac}{a_c}
\newcommand{\aPsi}{a_\Psi}
\newcommand{\am}{a_m}
\newcommand{\omgcut}{\omega_{\textup{cut}}}

\newcommand{\cD}{\mathscr{D}}
\newcommand{\cN}{\mathscr{N}}
\newcommand{\cH}{\mathscr{H}}
\newcommand{\cL}{\mathscr{L}}
\newcommand{\cS}{\mathscr{S}}
\newcommand{\cA}{\mathscr{A}}
%\newcommand{\ci}{\mathbbm{i}}
\newcommand{\ci}{\mathfrak{i}}

\newcommand{\dens}{{n}}
\newcommand{\NSM}{Strange Half-Metal}
\newcommand{\NSMab}{SHM}
\newcommand{\nsm}{strange half-metal}

\newcommand{\dtau}{\textup{d}\tau}
\newcommand{\de}{\textup{d}\varepsilon}
\newcommand{\iwn}{\ci\omega_n}
\newcommand{\wpl}{\omega^+}
\newcommand{\wn}{\omega_n}
\newcommand{\dt}{\textup{d}t}
\newcommand{\dw}{\textup{d}\omega}

\newcommand{\omitthis}[1]{\ifdefined\showomitedparts{#1}\fi}
%\newcommand{\changes}[1]{\textcolor{red}{#1}}
\newcommand{\changes}[1]{#1}
%\newcommand{\newadd}[1]{\protect{\brickred{#1}}}
\newcommand{\newadd}[1]{#1}
%-----------------------------------------------
%-----------------From SYK_notes----------------
\newcommand{\intd}[1]{\mathbf{d}#1}
\newcommand{\cd}{c^\dagger}
\newcommand{\psid}{\psi^\dagger}
\newcommand{\Psid}{\Psi^\dagger}
\newcommand{\deltau}{\partial_\tau}
\newcommand{\itimeint}[1]{\int\limits_0^\beta \mathrm{d}#1}
\newcommand{\myeqnref}[1]{eqn[\ref{#1}]}
%-----------------------------------------------
%-----------------From HD_SYK-------------------
\newcommand{\SYKq}{\textup{SYK}_q}
\newcommand{\NSYK}{N_{\textup{SYK}}}
\newcommand{\scdots}{{\tiny\cdots\normalsize}}
\newcommand{\cb}{\bar{c}}
\newcommand{\Psib}{\bar{\psi}}
\newcommand{\ek}{\varepsilon_{b,\mathbf{k}}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\Gkwn}{G_b(\iwn,\mathbf{k})}
\newcommand{\Gkw}{G_b(\omega,\mathbf{k})}
\newcommand{\Abkw}{\rho_b(\omega,\mathbf{k})}
\newcommand{\db}{\bar{d}}
\newcommand{\LHS}{\textup{LHS}}
\newcommand{\FOne}{\mathcal{F}^{\textup{(1)}}}
\newcommand{\FTwo}{\mathcal{F}^{\textup{(2)}}}
\newcommand{\Fi}{\mathcal{F}^{\textup{(i)}}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\KOO}{K^{\textup{(11)}}}
\newcommand{\KTT}{K^{\textup{(22)}}}
\newcommand{\KOT}{K^{\textup{(12)}}}
\newcommand{\KTO}{K^{\textup{(21)}}}
\newcommand{\Kintra}{\tilde{K}_{\textup{intra}}}
\newcommand{\Kinter}{\tilde{K}_{\textup{inter}}}
\newcommand{\Kzintra}{\tilde{K}_{\textup{intra}}^{(q=0)}}
\newcommand{\Kzinter}{\tilde{K}_{\textup{inter}}^{(q=0)}}
\newcommand{\MKzintra}{\mathbf{K}_{\textup{intra}}^{(q=0)}}
\newcommand{\MKzinter}{\mathbf{K}_{\textup{inter}}^{(q=0)}}
\newcommand{\lzintra}{\lambda_{\textup{L(intra)}}^{(\vtr{q}=\vtr{0})}}
\newcommand{\lzinter}{\lambda_{\textup{L(inter)}}^{(\vtr{q}=\vtr{0})}}
\newcommand{\lmax}{\lambda^{\textup{(M)}}_\textup{L}}
\newcommand{\vtr}[1]{\mathbf{#1}}
\newcommand{\Tr}{\textup{Tr}}
\newcommand{\NFL}{\textup{NFL}}
\newcommand{\LFL}{\textup{LFL}}
\newcommand{\act}{S_\textup{action}}
\renewcommand{\Im}{\mathrm{Im}}
\renewcommand{\Re}{\mathrm{Re}}
\newcommand{\Eqns}[1] {Eqns.~(\ref{#1})}
%------------------------------------------------
\newcommand{\dz}{\mathrm{d}z}
%\newcommand{\tbd}[1]{\textbf{#1}}
\newcommand{\tbd}[1]{}
\newcommand{\coT}{\mathcal{T}}
\newcommand{\rT}{\mathbf{t}}
\def\action{\mathcal{S}}
%\newcommand{\concept}[1]{#1}
\newcommand{\concept}[1]{}
\newcommand{\figconcept}[1]{}
%\newcommand{\figconcept}[1]{#1}
\newcommand{\eqnconcept}[1]{}
%\newcommand{\eqnconcept}[1]{#1}
\newcommand{\tabconcept}[1]{}
%\newcommand{\tabconcept}[1]{#1}
\newcommand{\appconcept}[1]{}
%\newcommand{\appconcept}[1]{#1}
\newcommand{\appcite}[1]{Appendix \ref{#1}}
%\newcommand{\appcite}[1]{appendix}
\newcommand{\tabcite}[1]{table.~\ref{#1}}
\def\ri{l}
\def\nR{R}
\def\pZ{\mathcal{Z}}
\newcommand{\chapcite}[1]{chap.~\ref{#1}}
\def\bi{band insulator}
\def\BI{Band Insulator}
\def\Bi{Band insulator}
\def\phiholo{\phi_\textup{holo}}
\def\Eholo{\vtr{E}_\textup{holo}}
\def\Efocus{\vtr{E}_\textup{focus}}
\def\cEfocus{\vtr{\tilde{E}}_\textup{focus}}
\def\cEholo{\vtr{\tilde{E}}_\textup{holo}}
\def\Ifocus{I_\textup{focus}}
\def\Itarget{I_\textup{target}}
\def\FT{\textup{FT}}
\def\IFT{\textup{FT}^{-1}}
\def\Ds{\Delta_\Sigma}
\def\fs{f}
\newcommand{\Sgn}[1]{\textup{Sgn}(#1)}
\newcommand{\eqns}[1]{eqns.(\ref{#1})}
\newcommand{\Nequation}[1]{Neqns.\ref{#1}}
\def\Tbkt{T_{\textup{BKT}}}
\def\mI{\mathbf{1}}

\def\vd{\vtr{d}}
\def\tmat{\mathbf{t_{\textup{hop}}}}
\def\abs{\textup{Abs}}
\def\Ebg{\Delta E_{bg}}
\def\VDW{V_{\mathrm{DW}}}
\def\kfree{\vtr{k}_{\textup{free}}}
\newcommand\op[1]{{\bf #1}}
\def\Vlat{V_{\textup{lat}}}
\def\Vconf{V_{\textup{conf}}}
\def\eC{\varepsilon_{\textup{C}}}
\def\eV{\varepsilon_{\textup{V}}}
\def\gn{\xi}
\def\HMF{H_{\textup{MF}}}
\def\Nk{N_{\vk}}
\def\Gpot{\Omega}
\def\Gpdens{\Xi}
\def\pZneq{Z_{neq}}
\def\vx{\vtr{x}}
\def\Srep{\action_{\textup{rep}}}
\def\DSig{\Delta_\Sigma}
\def\DSigs{\Delta_{\Sigma_s}}
\def\DSigc{\Delta_{\Sigma_s}}
\def\DSigPsi{\Delta_{\Sigma_\Psi}}
\def\zsw{z}
\def\FTVlat{\hat{V}_{\textup{lat}}}
\def\FTVDW{\hat{V}_{\textup{DW}}}
\def\TO{\textup{T}}
\def\ATO{\tilde{\textup{T}}}
\def\rhs{r.h.s}
\def\lhs{l.h.s}

\def\cTO{\mathcal{T}}
\def\cATO{\tilde{\mathcal{T}}}
\def\Zneq{\mathcal{Z}_\textup{neq}}
\def\ctimeint{\int_\mathcal{C}\textup{d}}

\newcommand{\cs}{{c^*}}
\newcommand{\psis}{{\psi^*}}
\newcommand{\Gcr}{{G_{r,r'}}^{(i)}(\tau,\tau')}
\newcommand{\Gcrrpt}{G_{\rt,\rt'}(i)}
\newcommand{\Gcrprt}{G_{\rt',\rt}(i)}
\newcommand{\Gpsi}{\mathcal{G}_i(\tau,\tau')}
\newcommand{\Gpsir}{{\mathcal{G}_{r,r'}}^{(i)}(\tau,\tau')}
\newcommand{\Gpsrrpt}{\mathcal{G}_{\rt,\rt'}(i)}
\newcommand{\Gpsrprt}{\mathcal{G}_{\rt',\rt}(i)}

\newcommand{\Srrpt}{\Sigma_{\rt,\rt'}(i)}
\newcommand{\Srprt}{\Sigma_{\rt',\rt}(i)}
\newcommand{\srrpt}{\sigma_{\rt,\rt'}(i)}
\newcommand{\srprt}{\sigma_{\rt',\rt}(i)}

\newcommand{\cI}{\mathfrak{i}}
\newcommand{\intpminf}{\int\limits_{-\infty}^\infty}
\newcommand{\dOmg}{\mathrm{d}\Omega}
\newcommand{\intzerobeta}{\int\limits_{0}^\beta\dtau}
\newcommand{\sumFMs}{\sum\limits_{\iwn}}
\newcommand{\G}[2]{G^{#2}_{#1}}
\newcommand{\iw}[1]{\mathfrak{i}\omega_{#1}}
\newcommand{\dint}[1]{\mathrm{d}{#1}}



\global\long\def\ren{S^{(n)}}

\global\long\def\retwo{S^{(2)}}

\global\long\def\ra{\rangle}

\global\long\def\la{\langle}

\global\long\def\rang{\rangle}

\global\long\def\lang{\langle}

\global\long\def\I{\mathbf{1}}

\def\del{\partial}

\usepackage{cancel}

